Spurious Features Everywhere -- Large-Scale Detection of Harmful Spurious Features in ImageNet

Benchmark performance of deep learning classifiers alone is not a reliable predictor for the performance of a deployed model. In particular, if the image classifier has picked up spurious features in the training data, its predictions can fail in unexpected ways. In this paper, we develop a framework that allows us to systematically identify spurious features in large datasets like ImageNet. It is based on our neural PCA components and their visualization. Previous work on spurious features often operates in toy settings or requires costly pixel-wise annotations. In contrast, we work with ImageNet and validate our results by showing that presence of the harmful spurious feature of a class alone is sufficient to trigger the prediction of that class. We introduce the novel dataset "Spurious ImageNet" which allows to measure the reliance of any ImageNet classifier on harmful spurious features. Moreover, we introduce SpuFix as a simple mitigation method to reduce the dependence of any ImageNet classifier on previously identified harmful spurious features without requiring additional labels or retraining of the model. We provide code and data at https://github.com/YanNeu/spurious_imagenet .

==> spurious_examples_4.tex <==
\begin{figure*}
    \setlength{\tabcolsep}{0.1em}
    \centering
    \normalsize
    \begin{tabular}{c c c c c p{0.02\textwidth} c c c c c}
        \multicolumn{5}{l}{{\blue\textbf{Hummingbird}} -  Random train. images (\textbf{confidence}\,\,/\,$\alpha_k$)} 
        &&\multicolumn{5}{c}{Images with spurious \textbf{bird feeder} but \textbf{no hummingbird}}\\ 
        {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/rand_train_img_1.jpg}} 
        &{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/rand_train_img_2.jpg}}
        &{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/rand_train_img_3.jpg}}
        &{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/rand_train_img_4.jpg}} 
        &{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/rand_train_img_5.jpg}}
        &&{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/bing_000050_cropped.jpg}}%
        &{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/pc_idx_1_img_5_-hummingbird_feeder-_bee.jpg}}
        &{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/pc_idx_1_img_4_-hummingbird_feeder-_bee.jpg}}
        &{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/14.png}}
        &{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/116.png}}\\
        $\mathbf{0.93}$\,/\,$1.7$
        &$\mathbf{1.00}$\,/\,$-0.9$
        &$\mathbf{0.96}$\,/\,$-1.0$
        &$\mathbf{0.99}$\,/\,$2.2$
        &$\mathbf{1.00}$\,/\,$1.54$
        &&$\mathbf{0.94}$\,/\,$5.7$
        &$\mathbf{0.94}$\,/\,$3.4$
        &$\mathbf{0.82}$\,/\,$2.9$ 
        &$\mathbf{0.91}$\,/\,$5.6$
        & $\mathbf{0.91}$\,/\,$4.7$\\
        \multicolumn{1}{c}{\NPFV} & \multicolumn{4}{c}{Maximally activating training images} && \multicolumn{5}{c}{all classified as \textbf{humming bird} by four ImageNet models}\\
        {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/cf_pc_1.jpg}}& 
        {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/act_pc_1_max_0.jpg}}&  {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/act_pc_1_max_1.jpg}}&  {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/act_pc_1_max_2.jpg}} &
        {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/act_pc_1_max_3.jpg}}&&
        {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/bing_hum_fee_000005.jpg}}&  {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/bing_000075_cropped.jpg}}&  {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/wiki_1.jpg}}&  {\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/wiki_4.jpeg}}&{\includegraphics[width=0.095\textwidth]{figures/img/hummingbird/wiki_3.jpg}}\\
        $\mathbf{1.00}$\,/\,$9.7$
        &$\mathbf{1.00}$\,/\,$7.5$
        &$\mathbf{1.00}$\,/\,$5.9$
        &$\mathbf{1.00}$\,/\,$5.6$
        &$\mathbf{1.00}$\,/\,$5.6$
        &&$\mathbf{0.86}$\,/\,$4.3$
        &$\mathbf{0.81}$\,/\,$3.5$
        &$\mathbf{0.89}$\,/\,$3.3$
        &$\mathbf{0.89}$\,/\,$3.8$
        &$\mathbf{0.78}$\,/\,$5.91$
    \end{tabular}
    \caption{\label{fig:spurious-exp} \textbf{Spurious features (ImageNet):} found by human labeling of our neural PCA components. For each class we show 5 random train. images (top left), the neural PCA Feature Visual. (NPFV) and 4 most activating train. images for the component with the spurious feature (bottom left). Right: all four ImageNet models classify images \textbf{only showing the spurious feature but not the class} as the class.} %
\end{figure*}
